Models for COVID-19 Pandemic: A Comparative Analysis

COVID-19 pandemic represents an unprecedented global health crisis in the last 100 years. Its economic, social and health impact continues to grow and is likely to end up as one of the worst global disasters since the 1918 pandemic and the World Wars. Mathematical models have played an important role in the ongoing crisis; they have been used to inform public policies and have been instrumental in many of the social distancing measures that were instituted worldwide. In this article we review some of the important mathematical models used to support the ongoing planning and response efforts. These models differ in their use, their mathematical form and their scope.

==> Bios.tex <==
\newpage
\section{Biographies}

\begin{wrapfigure}{r}{0.16\textwidth}
\vspace{-13pt}
\centering
\includegraphics[width=0.14\textwidth]{figs/aniruddha_adiga_webedited.jpg}
\end{wrapfigure}

Aniruddha Adiga is a Postdoctoral Research Associate at the NSSAC Division of the Biocomplexity Institute and initiative. He completed his PhD from the Department of Electrical Engineering, Indian Institute of Science (IISc), Bangalore, India and has held the position of Postdoctoral fellow at IISc and North Carolina State University, Raleigh, USA. 
His research areas include signal processing, machine learning, data mining, forecasting, big data analysis etc. At NSSAC, his primary focus has been the analysis and development of forecasting systems for epidemiological signals such as influenza-like illness and COVID-19 using auxiliary data sources.\\   

\begin{wrapfigure}{l}{0.18\textwidth}
\vspace{-10pt}
\centering
\includegraphics[width=0.16\textwidth]{figs/Devdatt_Dubhashi-3.jpg}
\end{wrapfigure}
\noindent
Devdatt Dubhashi is a Professor in the Data Science and AI Division in the Department of computer Science and Engineering, Chalmers University Sweden. His research interests are in machine learning, algorithms and cognitive science. 
He received his Ph.D. in Computer Science at Cornell University USA and has held positions at the Max Planck Institute for Computer Science, Saarbr\"ucken Germany, BRICS (Basic Research in computer Science) a center of the Danish National Science Foundation at the University of Aarhus Denmark and at the Indian Institute of Technology, Delhi India.\\

\begin{wrapfigure}{r}{0.15\textwidth}
\vspace{-14pt}
\centering
\includegraphics[width=0.13\textwidth]{figs/Bryan-Lews.png}
\end{wrapfigure}
Bryan Lewis is a research associate professor in the Network Systems Science and Advanced Computing division. His research has focused on understanding the transmission dynamics of infectious diseases within specific populations through both analysis and simulation. Lewis is a computational epidemiologist with more than 15 years of experience in crafting, analyzing, and interpreting the results of models in the context of real public health problems. As a computational epidemiologist, for more than a decade, Lewis has been heavily involved in a series of projects forecasting the spread of infectious disease as well as evaluating the response to them in support of the federal government. These projects have tackled diseases from Ebola to pandemic influenza and melioidosis to cholera.\\



\begin{wrapfigure}{l}{0.17\textwidth}
\vspace{-13pt}
\centering
\includegraphics[width=0.14\textwidth]{figs/Madhav-Picture-Feb2019.pdf}
\end{wrapfigure}
Madhav Marathe is a Distinguished Professor in 
Biocomplexity, the division director of the Networks, Simulation Science and Advanced Computing (NSSAC) Division at the Biocomplexity Institute and  
Initiative, and a Professor in the Department of Computer Science at the University of Virginia (UVA).  
His research interests are in network
science, computational epidemiology, AI, foundations of computing,
socially coupled system science and high performance computing. 
Before joining UVA, he held positions at Virginia Tech and  the Los Alamos National Laboratory. He is a Fellow of the IEEE, ACM, SIAM and AAAS.\\

\noindent
\begin{wrapfigure}{r}{0.15\textwidth}
\vspace{-13pt}
\centering
\includegraphics[width=0.13\textwidth]{figs/Srini_Headshot_2019.jpg}
\end{wrapfigure}
Srinivasan (Srini) Venkatramanan is a Research Scientist at the Biocomplexity Institute \& Initiative, University of Virginia and his research focuses on developing, analyzing and optimizing computational models in the field of network epidemiology. He received his PhD from the Department of Electrical and Communication Engineering, Indian Institute of Science (IISc), and did his postdoctoral research at Virginia Tech. His areas of interest include network science, stochastic modeling and big data analytics. He has used in-silico models of society to study the spread of infectious diseases and invasive species. Recent research includes modeling and forecasting emerging infectious disease outbreaks (e.g., Ebola, COVID-19), impact of human mobility on disease spread and resource allocation problems in the context of epidemic control (e.g., seasonal influenza vaccines). \\


\begin{wrapfigure}{l}{0.15\textwidth}
\vspace{-14pt}
\centering
\includegraphics[width=0.13\textwidth]{figs/anil.jpg}
\end{wrapfigure}
\medskip
\noindent
Anil Vullikanti is a Professor in the Biocomplexity Institute and the Department of Computer Science
at the University of Virginia. He got his PhD at the Indian Institute of Science, and was a postdoctoral associate at the Max Planck Institute for Computer Science, Saarbr\"ucken, Germany, and the Los Alamos National Lab. His research interests are in the broad areas of network science, dynamical systems, combinatorial optimization, and distributed computing, and their applications to computational epidemiology and social networks.

==> old-background.tex <==


We start with a very commonly used model, popularly known as the SIR model,
involving ordinary differential equations based on a mass-action assumption
(see \cite{Brauer-2008,Ne03, marathe:cacm13} for details).
A population of size $N$ is divided into three states:
susceptible ($S$), infective ($I$) and removed or recovered ($R$) (see Figure \ref{fig:sir}).
The following process describes the system dynamics:
each infected person can infect any susceptible person
(independently) with probability $\beta$, and can recover with probability $\gamma$.
Let $S(t)$, $I(t)$ and $R(t)$ denote the number of people who are
susceptible, infected and recovered states at time $t$, respectively.
Let $s(t)=S(t)/N$, $i(t)=I(t)/N$ and $r(t)=R(t)/N$; then,
$s(t)+i(t)+r(t)=1$. 
Under the ``complete mixing'' assumption that each individual is in contact with
everyone in the population, the system of differential equations in
Figure~\ref{fig:sir}(b) are used to describe the dynamics of the SIR model.

% \begin{figure}
% \begin{minipage}{0.65\textwidth}
% %\begin{figure}
% %\begin{center}
% %%%\includegraphics[width=0.6\linewidth]{figs/model-classification.pdf}
% \includegraphics[width=1.0\linewidth]{figs/sir-comp.pdf}
% %\label{fig:model-classification}
% %\end{center}
% %\end{figure}
% \end{minipage}
% \hspace*{-0.2in}
% \begin{minipage}{.30\textwidth}
% \begin{eqnarray*}
% \frac{ds}{dt} &=& -\beta is\\
% \frac{di}{dt} &=& \beta is - \gamma i\\
% \frac{dr}{dt} &=& \gamma i
% \end{eqnarray*}
% \end{minipage}
% \caption{The SIR model. (a) The entire population is split into compartments corresponding
% to the S, I and R states. Any two individuals in the population can come in contact.
% (b) Coupled differential equations for the SIR model.}
% \label{fig:sir}
% \end{figure}
\begin{figure}
    \centering
    \subfloat{\includegraphics[width=.8\textwidth]{figs/SIR model.pdf}\label{<figure1>}}
    \caption{The SIR model. (a) The entire population is split into compartments corresponding to the S, I and R states. Any two individuals in the population can come in contact. (b) Coupled differential equations for the SIR model.}
% \label{fig:sir}
\end{figure}


One of the classic results in the SIR model is that there is an epidemic
which infects a large fraction of the population, if and
only if $R_0=\beta/\gamma >1$ (see \cite{dimitrov:informs} for the derivation); 
$R_0$ is known as the ``reproductive number'', and
has been key in characterizing an epidemic. At the start of an epidemic, much of
the public health  effort is focused on estimating $R_0$ from observed 
infections \cite{lipsitch:science03}.
Further, public health decision making for controlling an epidemic is often
translated to reducing $R_0$---
this can be done in many ways, e.g., by reducing $\beta$ (through better protective
measures, such as washing and face masks, in the case of flu) \cite{dimitrov:informs}.
While the notion of $R_0$ has given a lot of insights into the spread of epidemics,
there are several limitations. For instance, during the SARS outbreak in 2003, the
$R_0$ was estimated to be in the range $[2.2, 3.6]$. However, despite its spread over
many countries, it did not cause a very large outbreak for multiple reasons. First, the 
$R_0$ estimates were based on infections in crowded hospital wards, where a complete mixing
assumption is reasonable. But this does not hold in other settings. Second, as the epidemic spread,
people altered their behavior and started mixing less, which is not taken into account
in the static definition of $R_0$.

There has been a lot of work in developing more complex compartmental models in order to
address some of these issues,
including stochastic models, multiple compartments to represent various subpopulations, branching
processes, chain-binomial models, etc., see \cite{Ne03,Brauer-2008} and the references therein.
Overall, compartmental models have been immensely successful over the last 100 years, and have
become a workhorse of mathematical epidemiology. They are relatively
easy to extend and quick to build, and can either be solved analytically or
numerically quite efficiently, building on the well developed theory of ODEs.

In contrast to compartmental models, {\em networked epidemiology} considers epidemic
spread on a specific undirected contact network $G(V,E)$ 
on a population $V$ -- each edge $e=(u,v)\in E$ implies that
individuals (also referred to as nodes) $u, v\in V$ come into contact\footnote{%
Note that though edge $e$ is
represented as a tuple $(u, v)$, it actually denotes the set $\{u, v\}$, as
is common in graph theory.}
Let $N(v)$ denote the set of neighbors of $v$. 
For instance, in the graph in Figure \ref{fig:network-ex}, we have $V=\{a, b, c, d\}$
and $E=\{(a, b), (a, c), (b, d), (c d)\}$. Node $a$ has $b$ and $c$ as neighbors, so $N(a)=\{b, c\}$.
The SIR model on the graph $G$ is a dynamical process in which
each node is in one of $S$, $I$ or $R$ states.  Infection can
potentially spread from $u$ to $v$ along edge $e=(u,v)$ with a probability of
$\beta(e,t)$ at time instant $t$
after $u$ becomes infected, conditional on node $v$ remaining uninfected
until time $t$--- this is a discrete version of the rate of infection for the
ODE model discussed earlier. 
We let $I(t)$ denote the set of nodes that become
infected at time $t$. 
The (random) subset of edges on which the infections spread represents
a disease outcome, and is referred to as a \emph{dendogram}.
This dynamical system starts with a configuration in which there are one or more nodes
in state {\sf I} and reaches a fixed point in which all nodes are in states {\sf S} or {\sf R}.
Figure \ref{fig:network-ex} shows an example of the SIR model on a network.

\begin{figure*}
\begin{center}
\includegraphics[width=0.5\linewidth]{figs/sir-nw.pdf}
%\vspace{-0.23in}
\caption{The SIR process on a graph. The contact graph $G=(V, E)$ is defined on
a population $V=\{a, b, c, d\}$. The node colors white, black and grey represent
the Susceptible, Infected and Recovered states, respectively. Initially, only node $a$
is infected, and all other nodes are susceptible. A possible outcome at $t=1$
is shown, in which node $c$ becomes infected, while node $a$ recovers. Node $a$ tries
to independently infect both its neighbors $b$ and $c$, but only node $c$ gets
infected--- this is indictated by the solid edge $(a, c)$.
The probability of getting
this outcome is $(1-p(a,b))p(a,c)$.}
\label{fig:network-ex}
\end{center}
\end{figure*}

The time series $(|I(t)|, t=0, 1,\ldots)$ is referred to as an \emph{epidemic curve} corresponding
to a stochastic outcome; this is a very commonly used quantity related to an epidemic.
The \emph{total number of infections} for an outcome is given by $\sum_t |I(t)|$.
The \emph{peak value} is $\max_t |I(t)|$, while the \emph{time to peak}
is the largest time $t$ that maximizes $|I(t)|$. These quantities are illustrated in
Figure \ref{fig:epicurve}. Also observe that the epicurve is not very smooth; this is in contrast
with the epicurve in an ODE model.
A popular variant of the SIR model is the SIS model, in which an infected node
switches to state {\sf S} after the infectious duration.  

\begin{figure*}
\begin{center}
\includegraphics[width=0.5\linewidth]{figs/epicurve.pdf}
\caption{Different quantities associated with the dynamics of epidemics. See discussion
in Section \ref{sec:models} for definitions of these quantities.}
\label{fig:epicurve}
\end{center}
\end{figure*}

Such a network model captures the interplay between the three components of 
computational epidemiology: (i) individual behaviors of agents, 
(ii) unstructured, heterogeneous multi-scale networks, 
and (iii) the dynamical processes on these networks.
It is based on the hypothesis that a better understanding of the
characteristics of the underlying network and individual behavioral
adaptation can give better insights into contagion dynamics and
response strategies.
Although computationally expensive and data intensive, network-based epidemiology
alters the types of questions that can be posed, providing
qualitatively different insights into disease dynamics and public health policies.
It also allows policy makers to formulate
and investigate potentially novel and context specific  interventions. 


==> old-results.tex <==

\section{Models from the Imperial College Modeling Group}
\label{sec:imperial}
\noindent
\textbf{Background.} \ The modeling group led by Neil Ferguson
was to our knowledge the first model to study the  impact of 
COVID-19 across two large countries: US and UK. 
The basic model was first developed in 2005 -- it was used to inform
policy pertaining to H5N1 pandemic and was one of three models used
to informal the federal pandemic influenza plan and led to the now well
accepted targeted layered containment (TLC) strategy. It was adopted to COVID-19 as discussed below.

\noindent
\textbf{Model Structure.} \ The basic model structure consists of 
developing a set of households based on census information for a given country. Individual members of the household interact with other members
of the household. The data to produce these households is obtained using Census information for these countries. The paper is not clear if a
national census is used or more detailed state wise census information is used. Schools, workplaces and random meeting points are then added.
The number of schools, workplaces and random meeting points are used to represent the potential places of interaction between individuals. 
Census data is used to assign age and household sizes.  
Data on average class sizes and staff-student ratios were used to generate a synthetic population of schools distributed proportional to local population density. Data on the distribution of workplace size was used to generate workplaces with commuting distance data used to locate workplaces appropriately across the population. Individuals are assigned to each of these locations at the start of the simulation. The gravity style kernel is used to decide how far a person can go in terms of attending
work, school or community interaction place. The number of contacts between individuals at school, work and community meeting points are calibrated to produce a given attack rate.

Each individual has an associated disease transmission model. The disease
transmission model parameters are based on data collected when the pandemic
was evolving in Wuhan; see page 4 of \cite{ferguson-report9}.

Finally, the model also has rich set of interventions. These include:
($i$) case isolation, ($ii$) voluntary home quarantine, ($iii$) Social distancing of those over 70 years, ($iv$) social distancing of the entire population, ($v$) closure of schools and universities; see page 6 \cite{ferguson-report9}. The code hsa now been available but the details of how such interventions are implemented remains a bit unclear. This is important as the interpretation of these interventions can have substantial
impact on the outcome.

\noindent
\textbf{What did the model suggest.} \ 
The Imperial college (IC Model) model was one of the first models to evaluate the COVID-19 pandemic using detailed agent-based model. The predictions made by the model were quite dire. The results show that to be able to reduce $R$ to close to 1 or below, a combination of case isolation, social distancing of the entire population and either household quarantine or school and university closure are required.  The model had tremendous impact --
UK and US both decide to start considering complete lock downs -- a
policy that was practically impossible to even talk about earlier in Western world. The paper came out around the same time that Wuhan epidemic was raging and the epidemic in Italy had taken the turn for the worse. This made the
model results even more critical. So far the numbers have not played out per model forecasts -- this is a general issue that we will discuss across all models.

\noindent
\textbf{Strengths and Limitations.} \
IC model was one of the first model by a very reputed group to report the
potential impact of COVID-19 with and without interventions. The model
was far more detailed than other models that were published by then.
The authors also took great care parameterizing the model with the best disease transmission data that was available until then. The model also considered a very rich set of interventions and was one of the first to analyze pulsing intervention. The work also had a few weaknesses. The
representation of the underlying social contact network was relatively 
simple. Second, the details of how interventions were represented were
not made clear. Since then the modelers have made their code open and
the research community has witnessed an intense debate on the pros and cons of various modeling assumptions and the resulting software system. 
We believe that despite some criticisms that were valid, overall the results
represented a breakthrough in terms of when the results were put out and
the level of details the model had. 

\section{Spatial metapopulation models}
\label{sec:metapop}

\noindent
\textbf{Background.}
This approach is an alternative to detailed agent based models, and has been used in
modeling the spread of multiple diseases, including Influenza~\cite{balcan:pnas2009, srini:ploscb19},
Ebola~\cite{gomes:plos-curr14} and Zika~\cite{zhang:pnas17}. It has been adapted for
studying the importation risk of SARS-CoV-2 across the world~\cite{chinazzi:science20}.
Structured metapopulation models construct a simple abstraction of the mixing patterns in the population,
in which the entire plane is decomposed into fully connected geographical regions,
representing subpopulation, which are connected through airline and commuter flow networks.
Thus, they lack the rich detail of agent based models, but have fewer parameters, and
are therefore, easy to set up and scale to large regions.

\noindent
\textbf{Model structure.}
Here, we summarize GLEaM~\cite{balcan:pnas2009} and PatchSim~\cite{srini:ploscb19}.
GLEaM uses two classes of datasets-- population estimates and mobility.
Population data is used from the ``Gridded Population of the World''~\cite{ciesin}, which
gives an estimated population value at a $15\times 15$ minutes of arc (referred
to as a ``cell'') over the entire planet.
Two different kinds of mobility processes are considered-- airline travel and commuter flow.
The former captures long-distance travel, whereas the latter captures localized mobility.
Airline data is obtained from the International Air Transport Association (IATA)~\cite{iata}, and
the Official Airline Guide (OAG)~\cite{oag}. There are about 3300 airports world-wide; these
are aggregated at the level of urban regions served by multiple airport (e.g., as in London).
A voronoi tesselation is constructed with the resulting airport locations as centers, and
the population cells are assigned to these cells, with a 200 mile cutoff from the center.
The commuter flows connect cells at a much smaller spatial scale.
We represent this mobility pattern as a directed graph on the cells, and refer to it
as the mobility network.

In the basic SEIR model, the subpopulation in each cell $j$ is partitioned into 
compartments $S_j, E_j, I_j$ and $R_j$, corresponding to the disease states.
For each cell $j$, we define
the force of infection $\lambda_j$ as the rate at which a susceptible individual in the
subpopulation in cell $j$ becomes infected---this is determined by the interactions the
person has with infectious individuals in cell $j$ or any cell $j'$ connected in the mobility network.
An individual in the susceptible compartment $S_j$ becomes infected with probability
$\lambda_j\Delta t$ and enters the compartment $E_j$, in a time interval $\Delta t$.
From this compartment, the individual moves to the $I_j$ and then the $R_j$ compartments,
with appropriate probabilities, corresponding to the diease model parameters.

The PatchSim~\cite{srini:ploscb19} model has a similar structure, except that it uses
administrative boundaries (e.g., counties), instead of
a voronoi tesselation, which are connected using the mobility network. Further, the disease model
is deterministic, i.e., the transitions across the compartments occur at fixed rates.

\noindent
\textbf{What did the models suggest?}

\noindent
\textbf{Strength and limitations.}
Structured metapopulation models provide a good tradeoff between the power and realism of
detailed agent-based models, and simplicity and need for fewer inputs for modeling,
and scalability. This is especially true in the early days of the outbreak, when the disease dynamics are
driven to a large extent by mobility, which can be captured more easily within such models,
and there is significant uncertainty in the disease model parameters.
However, once the outbreak has spread, it is harder to model detailed interventions
(e.g., social distancing), which are much more localized, and hard to model by a single parameter.


\section{Models in Sweden}
\label{sec:sweden-models}
Sweden was an outlier amongst countries in that it decided to implement public health interventions without a lockdown. Schools and universities were not closed and restaurants and bars remained open. Instead Swedish citizens
implemented "work from home" policies where possible.Moderate social distancing based on individual responsibility and without police enforcement was employed but emphasis was attempted to be placed on shielding the over 65 age group.

\subsection{Simple model}

\textbf{Background.} \ 
Statistician Tom Britton developed a very simple model with a  focus  on predicting the number of infected over time in Stockholm.

\noindent
\textbf{Model structure.} \ 
Britton \cite{Britton2020} used a very simple SIR General epidemic model. It is used to make a coarse grain prediction of the behaviour of the outbreak based on knowing the basic reproduction number $R_0$  and the doubling time $d$ in the initial phase of the epidemic. Calibration to calendar time was done using the observed number of case fatalities, together with estimates of the time between infection to death, and the infection fatality risk. Predictions were made assuming no change of behaviour, as well as for the situation where preventive measures are put in place at one specific time--point. 

\noindent
\textbf{What did the model suggest.} \ One of the controversial predictions from this model was that the number of infections in the Stockholm area would quickly rise towards attaining \emph{herd immunity} within a short period. However, mass testing carried out in Stockholm during June indicated a far smaller percentage of infections.

\noindent
\textbf{Strength and Limitations.} \ 
Britton's model was intended as a quick and simple method to estimate and predict an on-going epidemic outbreak both with and without preventive measures put in place. It was intended as a complement to more realistic and detailed modelling. The estimation-prediction methodology is much simpler and straight- forward to implement for this simple model. It is more transparent to see how the few model assumptions affect the results, and it is easy to vary the few parameters to see their effect on predictions so one could see which parameter- uncertainties have biggest impact on predictions, and which parameter-uncertainties are less influential.

\subsection{Compartmentalized Models}

\noindent
\textbf{Background.} \ 
A group around statistician Joacim Rockl\"ov developed a model to estimate the impact of COVID-19 on the Swedish population at the municipality level, considering demography and
human mobility under various scenarios of mitigation and suppression. They attempted to estimate the
time course of infections, health care needs, and the mortality in relation to the Swedish ICU capacity, as well as the costs of care, and compared alternative policies and counterfactual
scenarios.

\noindent
\textbf{Model structure.} \ \cite{Rocklov2020} used a SEIR compartmentalized model with age structured compartments (0-59, 60-79, 80+) susceptibles, infected, in-patient carem, ICU and recovered populations based on Swedish population data at the municipal level. It also incorporated inter-municipality travel using a radiation model. Parameters were calibrated based on a combination of values available from international literature and fitting to available outbreak data. The effect of a number of different intervention strategies were considered ranging from no intervention to modest social distancing and finally to imposed isolation of various groups. 

\noindent
\textbf{What did the model suggest.} \ 
The model predicted an estimated death toll of around 40,000 for the strategies based only on social distancing and between 5000 and 8000 for policies imposing stricter isolation. It predicted ICU cases of upto 10,000 without much intervention and upto 6000 with modest social distancing, way above the available capacity of about 500 ICU beds. 
\noindent
\textbf{Strength and limitations.} \ 
The model showed a good fit against the reported COVID-19 related deaths in Sweden up to 20th of April, 2020,
However, the predictions of the total deaths and ICU demand turned out to be way off the mark.

\subsection{Agent Based microsimulations}

\noindent
\textbf{Background.} \ 
Finally, \cite{Gardner2020}used an individual-based model parameterized on Swedish demographics to assess the anticipated spread of COVID-19.
\noindent
\textbf{model structure.} \ 
\cite{Gardner2020} employed the individual agent-based model based on work by Ferguson et al \cite{Ferg20}. Individuals are randomly assigned an age based on Swedish
demographic data and they are also assigned a household. Household size is normally distributed around the average household size in Sweden in 2018, 2.2 people per household. Households placed on a lattice using high-resolution population data from Landscan and census dara from the Statstics Sweden and each household is additionally allocated to a city based on
the closest city centre by distance and to a county based on city designation. Each individual is placed in a school or workplace at a rate similar to the current participation
in Sweden.

Transmission between individuals occurs through contact at each
individual's workplace or school, within their household, and in their communities. Infectiousness is thus a property dependent on contacts from household members,
school/workplace members and community members with a probability based on household distances. Transmissibility was calibrated against data for the period 21
March – 6 April to reproduce either the doubling time reported using pan-European data35 or the growth in reported Swedish deaths for that period

Various types of interventions were studied including the policy implemented in Sweden by the public health authorities as well as more aggressive interventions approaching full lockdown.

\noindent
\textbf{What did the model suggest.} \ 
Their prediction was that "under conservative epidemiological parameter estimates, the current Swedish public-health strategy will result in a peak intensive-care load in May that exceeds pre-pandemic capacity by over 40-fold, with a median mortality of 96,000 (95\% CI 52,000 to 183,000)". 

\noindent
\textbf{Strength and limitations.} \ 
This model was based on adapting the well known Imperial model discussed in section~\ref{sec:imperial} to Sweden and considered a wide range of intervention strategies. Unfortunately the predictions of the model were woefully off the mark on both counts: the deaths by June 18 are under 5000 and at he peak the ICU infrastructure had at least 20\% unutilized capacity.
\section{Forecasting Models}
In the US, the Centers for Disease Control and Prevention (CDC) provides 1-,2-,3-, and 4-week ahead forecasts on cumulative deaths at the national level and across all states. The forecasts are provided by 21 (as of June 24, 2020) modelling groups and the CDC reports the cumulative deaths based on an ensemble of these forecasts.
\subsection{COVID-19 ForecastHub}
\noindent
\textbf{Model structure} It has been observed previously in the case of other infectious disease that an ensemble of forecasts from multiple models tends to be better than any individual contributing model \cite{yamana2017individual}. Most of the models considered in the COVID-19 ForecastHub are variants of the SIER model with two models relying on agent-based models and one deep-learning-based model. The simulation outcomes are heavily dependent on the intervention scenarios considered. Some models assume that the effects of the interventions are reflected in the observed data and do not explicitly encode it in the model. Models such as [] incorporate the effects of interventions by suitably varying the contact rate while models [IHME,] incorporate the change in mobility patterns to reflect in the simulations. The current ensemble model equally weight the submitted forecasts.   
